Sparse projections onto the simplex

Most learning methods with rank or sparsity constraints use convex relaxations, which lead to optimization with the nuclear norm or the $\ell_1$-norm. However, several important learning applications cannot benefit from this approach as they feature these convex norms as constraints in addition to the non-convex rank and sparsity constraints. In this setting, we derive efficient sparse projections onto the simplex and its extension, and illustrate how to use them to solve high-dimensional learning problems in quantum tomography, sparse density estimation and portfolio selection with non-convex constraints.

==> applications.tex <==
\section{Sparse projectors in action}


\input{quantum}

\input{measurelearn}

\input{portfolio}


==> experiments.tex <==
\section{Experiments}\label{sec:experiments}
\subsection{Quantum tomography}
The ability to project onto trace and rank constraints allows us to formulate quantum state recovery problems that lead to better recovery. 
We follow the approach of \cite{QuantumTomoPRL} and generate random Pauli measurements and add white noise, which is suitably realistic to demonstrate the characteristics of recovery algorithms. The experiments that follow use a $8$ qubit system ($d=2^8$) with noise SNR at $30$~dB (so the absolute noise level changes depending on the number of measurements), and a $7$ qubit noiseless system.

The measurements are generated using a random real-valued matrix $\X^\star$ with rank $2$, although the algorithms also work with complex-valued matrices. A $d\times d$ rank $r$ real-valued matrix has $dr-r(r-1)/2 \approx dr$ degrees of freedom, so this is a lower bound on the number of measurements needed to recover $\X^\star$ from noiseless measurements. To test the various approaches, we vary the number of measurements between $2dr$ and $5dr$. We assume $r$ is known, though other computational experience suggests that estimates of $r$ return good answers as well.
% N.B. The algo take advantage of the realness for their projections.

The convex problem~\eqref{eq:conventional} depends on a parameter $\lambda$. We solve the problem for different $\lambda$ in a bracketing search until we find the first $\lambda$ that provides a solution with numerical rank $r$ (i.e., only $r$ eigenvalues are larger than $10^{6}$), and then normalize this final solution to have trace $1$. Additionally, we test the following convex approach:
\begin{equation} \label{eq:conventional_2}
    \minimize_{ \X \succeq 0, \|\X\|_* \le 1} \|\linmap(\X) - \obs\|_F^2.
\end{equation}
Compared to~\eqref{eq:conventional}, no parameters are needed since we exploit prior knowledge of the trace, but there is no guarantee on the rank.  Both convex approaches can be solved with proximal gradient descent; we use the TFOCS package~\cite{becker2010templates} since it uses a sophisticated line search and Nesterov acceleration.

To illustrate the power of the combinatorial projections, we also solve the following non-convex formulation:
\begin{equation} \label{eq:quantum_nonconvex}
    \minimize_{ \X \succeq 0, \|\X\|_* \le 1, \text{rank}(\X)=r} \|\linmap(\X) - \obs\|_F^2.
\end{equation}
Using the projected gradient algorithm~\eqref{eq: projected gradient}, each step of the algorithm is a GSSP problem. The stepsize is $\mu^i=3/\|\linmap\|^2$ where $\|\cdot\|$ is the operator norm; it is also possible to use Nesterov acceleration to speed convergence, but we use~\eqref{eq: projected gradient} for simplicity. Due to the non-convexity, the algorithm depends on the starting value $\X_0$. We try two strategies: $(i)$ random initialization, and $(ii)$ initializing with the solution from~\eqref{eq:conventional_2}. In many cases, both initializations lead to the same stationary point.

Figure~\ref{fig:quantum1} shows the relative error $\|\X-\X^\star\|_F/\|\X^\star\|_F$ of the different approaches. All approaches do poorly when there are only $2dr$ measurements since this is near the noiseless information-theoretic limit. For higher numbers of measurements, the non-convex approach substantially outperforms both convex approaches. For $2.4dr$ measurements, it helps to start $\X_0$ with the convex solution, but otherwise the two non-convex approaches are nearly identical, which is likely because the number of local minima decreases as the number of rows of $\linmap$ increases. Between the two convex solutions, \eqref{eq:conventional} outperforms \eqref{eq:conventional_2} since it tunes $\lambda$ to achieve a rank $r$ solution. Neither convex approach is competitive with the non-convex approaches since they do not take advantage of the prior knowledge on trace and rank.  Figure~\ref{fig:quantum2} shows more results on a $7$ qubit problem with noiseless measurements. Again, the non-convex approach gives better results, particularly when there are fewer measurements. As expected, both approaches approach perfect recovery as the number of measurements increases.
%Describe the time, but don't plot.
%It would be nice to have information on ranks for the 2nd convex approach.

Another benefit to the non-convex approach is that the number of eigenvectors needed in the partial eigenvalue decomposition is at most $r$, whereas the convex approach may have intermediate iterates of arbitrarily high iteration, especially during the first few iterations. Table~\ref{tab:quantum} shows time per iteration for the convex and non-convex approach (overall time is more complicated, since the number of iterations depends on linesearch and other factors). Even using Matlab's dense eigenvalue solver \verb@eig@, the iterations of the non-convex approach are faster; problems that used an iterative Krylov subspace solver would show an even larger discrepancy.\footnote{Quantum state tomography does not benefit from using iterative eigenvalue solvers, since the range of $\linmap^*$ is not sparse.}

\begin{figure}
    \centering
    \includegraphics[width=.7\linewidth]{quantum_simplexPaper_8qubits_10rep}
    %\includegraphics[width=.8\linewidth]{quantum_simplexPaper_7qubits_15rep}
    \caption{Comparing the convex and non-convex approaches for quantum state tomography, $8$ qubits, $30$~dB SNR.
    Each point is the median over 10 runs of different random problems. % for 8 qubit
    %Each point is the median over 15 runs of different random problems. % for 7 qubit
    Convex approach $1$ refers to~\eqref{eq:conventional} and approach $2$ is~\eqref{eq:conventional_2}.}
    \label{fig:quantum1}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=.7\linewidth]{quantum_simplexPaper_7qubits_10rep_noiseless}
    \caption{Same as Figure~\ref{fig:quantum1} but with $7$ qubits, no noise. }
    \label{fig:quantum2}
\end{figure}

\begin{table}
    \centering
    \begin{tabular}{lcc}
        \toprule % use booktabs package
        Approach & mean time & standard deviation \\
        \midrule
        convex & $0.294$~s. & $0.030$~s. \\
        non-convex & $0.192$~s. & $0.019$~s. \\
        \bottomrule
    \end{tabular}
    \caption{Time per iteration of convex and non-convex approaches for quantum state tomography with $8$ qubits.}
    \label{tab:quantum}
\end{table}

\subsection{Density learning}
\begin{figure*}
   \begin{minipage}[t]{0.33\textwidth}
      \vspace{0pt}
      \includegraphics[width=\linewidth]{pdf1-crop}
	  %\begin{center} (a) \end{center}
   \end{minipage}
   \begin{minipage}[t]{0.33\textwidth}
      \vspace{0pt}
      \includegraphics[width=\linewidth]{pdf2-crop}
	  %\begin{center} (a) \end{center}
   \end{minipage}
   \begin{minipage}[t]{0.33\textwidth}
      \vspace{0pt}
      \includegraphics[width=\linewidth]{pdf3-crop}
	  %\begin{center} (a) \end{center}
   \end{minipage}
   \caption{\small\sl
Density estimation results using the Parzen window method, the quadratic programming in \eqref{eq:SDE} and our approach for $\sparsity = 5$.} \label{fig: Exp6}
\end{figure*}

\begin{figure*}
   \begin{minipage}[t]{0.24\textwidth}
      \vspace{0pt}
      \subfigure[$\sparsity = 3$]{\includegraphics[width=\linewidth]{pdf4-crop}}
	  %\begin{center} (a) \end{center}
   \end{minipage}
   \begin{minipage}[t]{0.24\textwidth}
      \vspace{0pt}
      \subfigure[$\sparsity = 8$]{\includegraphics[width=\linewidth]{pdf5-crop}}
	  %\begin{center} (a) \end{center}
   \end{minipage}
   \begin{minipage}[t]{0.24\textwidth}
      \vspace{0pt}
      \subfigure[$\sparsity = 10$]{\includegraphics[width=\linewidth]{pdf6-crop}}
	  %\begin{center} (a) \end{center}
   \end{minipage}
   \begin{minipage}[t]{0.24\textwidth}
      \vspace{0pt}
      \subfigure[$\sparsity = 15$]{\includegraphics[width=\linewidth]{pdf7-crop}}
	  %\begin{center} (a) \end{center}
   \end{minipage}
   \caption{\small\sl
Density estimation results for various sparsity levels $\sparsity$. Red spikes depict the estimated kernel means as well as the their relative contribution to the Gaussian mixture. As $\sparsity$ increases, the additional nonzero coefficients in $\bestsignal$ tend to have small weights.} \label{fig: Exp7}
\end{figure*}

\textbf{Sparse estimation of Gaussian mixtures:} We consider the following one-dimensional mixture of $5$ Gaussians: $f(x) = \frac{1}{5}\sum_{i = 1}^5 \kappa_{\sigma_i}(\signal_i, x)$ where $\sigma_i = (7/9)^i$ and $\signal_i = 14(\sigma_i - 1)$. A sample of $1000$ points is drawn from $f(x)$. We compare the density estimation performance of: $(i)$ the Parzen window method \cite{parzen1962estimation}, $(ii)$ the quadratic programming formulation in \eqref{eq:SDE}, and $(iii)$ our cardinality-constrained version of \eqref{eq:SDE} using GSSP. While $f(x)$ is constructed by kernels with various widths, we assume a constant width during the kernel estimation. In practice, the width is not known {\em a priori} but can be found using cross-validation techniques, i.e., leave-one-out technique; for simplicity, we assume kernels with width $\sigma = 1$.

Figure \ref{fig: Exp6}(a) depicts the true pdf and the estimated densities using the Parzen window method and the quadratic programming approach. Moreover, the figure also include a scaled plot of $1/\sigma_i$, indicating the height of the individual Gaussian mixtures. By default, the Parzen window method estimation interpolates $1000$ Gaussian kernels with centers around the sampled points to compute the estimate $\hat{f}(x)$; unfortunately, neither the quadratic programming approach (as Figure \ref{fig: Exp6}(b) illustrates) nor the Parzen window estimator results are easily {\it interpretable}  while both approaches provide a good approximation of the true pdf.

In stark contrast, using our cardinality-constrained approach, we can significantly enhance the interpretability. This is because the sparsity-constrained approach approximately reveals the number of Gaussian components. To see this, we first show the coefficient profile of the sparsity based approach $(iii)$ for $\sparsity = 5$ in Figure \ref{fig: Exp6}(b) (middle-bottom). Moreover, Figure \ref{fig: Exp6}(c) shows the estimated pdf for $\sparsity = 5$ along with the positions of weight coefficients obtained by our sparsity enforcing approach. Note that most of the weights obtained concentrate around the true means, providing some prior information about the ingredients of $f(x)$---this happens with rather high frequency in the experiments we conducted. Figure \ref{fig: Exp7} illustrates further estimated pdf's using our approach for various $\sparsity$. From the plot, it is also clear that if $k>5$, the resulting solutions are still approximately 5-sparse as the over estimated coefficients exhibit extremely small values.

% ---------------------------------------------------------
\subsection{Sparse measure learning}
\srb{Not sure where to put this section -- maybe earlier, if we want to link it with Non-parameteric estimation in 6.2 ?}

We follow the approach of \cite{pilanci2012recovery} and seek an estimate $\widehat{\signal}$ of a sparse discrete probability measure $\signal\in \R^\dimension$ which is indirectly observed by observing the moments of random variables $\mathbb{E}_{\signal}[X_i] = y_i$, $i=1,\ldots,m$.
Collecting the observations in the linear equation $\linmap(\signal) = \obs$, we have the following problem:
\begin{equation}
    \text{find}_{\signal\in\R^\dimension} \quad\text{subject to}\quad \signal\in\Delta_1^+,\quad \linmap(\signal) = \obs
    \label{eq:sparseMeasure}
\end{equation}
For $m \ll \dimension$, \eqref{eq:sparseMeasure} has many solutions. The basis pursuit solution first minimizes $\|\signal\|_1$ subject to $\signal \ge 0$ and $\linmap(\signal)= \obs$, and then renormalizes $\signal$ to enforce $\signal\in\Delta^+$. One possible greedy approach is to minimize $\|\linmap(\signal) -\obs\|^2$ subject to $\signal \in \Delta_1^+ \cap \Sigma_\sparsity$ for some sparsity level $\sparsity$, which we can solve using \eqref{eq: projected gradient} and the GSSP.

To provide a comparison with the greedy approach, we test 
the method of \cite{pilanci2012recovery}, 
which recovers sparse solutions to convex programs on the simplex by solving the convex program $\dimension$ times (as opposed to ${\dimension \choose \sparsity}\approx \dimension^\sparsity$ small problems for direct enumeration of all $\sparsity$-sparse solutions). The key observation is that the bound $|\text{supp}(x)| \ge \|x\|_1/\|x\|_\infty $, is simplified to $|\text{supp}(x)| \ge 1/\max_i(x_i)$ when $x \in \Delta_1^+$.
It is then possible to solve $\dimension$ problems (each with a different estimate $\hat{i}$ for $\argmax_i(x_i)$) and lower-bound the original
sparsity-regularized problem.  

\begin{figure}[h]
\centering
\includegraphics[width=.7\linewidth]{NoiselessData_MultipleApproaches_Error}
\includegraphics[width=.705\linewidth]{NoiselessData_MultipleApproaches_Time}
\caption{(Top) Comparison of sparse measure learning approaches as a function of $m/\dimension$. The greedy approach \eqref{eq: projected gradient} using the GSSP runs on problems of size $\dimension=10,\!000$ ($15$ runs). The other approaches use $\dimension=100$ ($25$ runs).  
(Bottom) Median solver time for $n=10,\!000$ (greedy) and $n=100$ (other approaches).}
    \label{fig:SparseKernel}
\end{figure}

Figure~\ref{fig:SparseKernel} shows accuracy and timing information of the methods on randomly generated problems. The greedy method scales well, so it was tested on problems of dimension $\dimension=10,\!000$ with sparsity $\sparsity=400$. Depending on the application, the sparsity may or may not be known \emph{a priori}. We test using the true sparsity parameter $400$ and also using $410$ (which returns nearly identical results). 
We note that in the presence of noise, the convex methods also require parameter estimates, so a test without noise is favorable to them.
%An accurate estimate of the parameter is not unreasonable: in the noisy case, 

The other approaches use $\dimension=100$ and $\sparsity=4$. In this low-dimensional setting, the phase transition (top figure) is not expected to be well-defined and it is hard to extrapolate to higher dimensions, but we see that direct enumeration works perfectly and the method of \cite{pilanci2012recovery} also works quite well, beating the simple convex approach.
The lower plot shows the median solver time; the greedy method on $\dimension=10,\!000$ is faster than all but the simplex convex approach for $\dimension=100$. The direct enumeration method scales extremely poorly, as expected (for $\dimension=50$, it was actually the fastest method, but for $\dimension=100$ it is the slowest method).

\subsection{?}
\tasos{Somehow, we have to connect this with the application description in the previous section}

For this case, we perform experiments on synthetic data. To simplify our case, we generate noiseless data according to $\obs = {\bf X} \bestsignal$ where $ \bestsignal \in \mathbb{R}^{2000} $ such that $\bestsignal \in \Delta_0$ and $\vectornorm{\bestsignal}_0 = s$ for $s = 200$. Here, ${\bf X} \in \mathbb{R}^{m \times 2000}$ is a column-normalized Gaussian matrix with iid entries for $m \in [600:100:1200]$ in \textsc{Matlab} notation. For each problem configuration, we perform 30 independent Monte-Carlo realizations. We set the tolerance accuracy to $10^{-10}$ for (\ref{eq:BP}) and $10^{-5}$ for the rest of the algorithms. We fix the maximum number of iterations to $3000$.

Given the above, we consider three optimization criteria: $(i)$ data fidelity squared-loss optimization over $\Sigma_s \cap \Delta_0$ constraint:
\begin{equation} \label{eq:data_fidelity_sparse_simplex}
    \minimize_{\signal \in \Sigma_s \cap \Delta_0} \|{\bf X} \signal - \obs\|_2^2, 
\end{equation} using \eqref{eq: projected gradient}, $(ii)$ data fidelity squared-loss optimization over $\Sigma_s$ constraint where the hyperplane constraint is included in the objective as follows:
\begin{equation} \label{eq:reg_data_fidelity_sparse_simplex}
    \minimize_{\signal \in \Sigma_s} \Big\|\begin{bmatrix}
    {\bf X} \\ \ones^T 
    \end{bmatrix}  
    \signal 
    - \begin{bmatrix} \obs \\  0 \end{bmatrix} \Big\|_2^2,
\end{equation} and, $(iii)$ basis pursuit method such that:
\begin{equation} \label{eq:BP}
    \minimize \vectornorm{\signal}_1~~\text{s.t.}~~\begin{bmatrix}
    {\bf X} \\ \ones^T 
    \end{bmatrix}  
    \signal 
    = \begin{bmatrix} \obs \\  0 \end{bmatrix}
\end{equation}

In figure \ref{fig:SparseHyper}, we show the relative error $\vectornorm{\widehat{\signal} - \bestsignal}_2 / \vectornorm{\bestsignal}_2$ for the three cases described above. We easily observe that the proposed {\it joint} projection scheme outperforms its regularized counterpart as long as the convex BP version in terms of the relative reconstruction error as the number of avaliable measurements decreases. We note that while (\ref{eq:data_fidelity_sparse_simplex})-(\ref{eq:reg_data_fidelity_sparse_simplex}) return sparse solutions, i.e., $\vectornorm{\widehat{\signal}}_0 = s$, BP approach returns a {\it fully dense} solution; thus, a heuristic postprocessing on the solution is needed to obtain sparse solutions. Moreover, the simple gradient scheme in \eqref{eq: projected gradient} is faster compared to the convex counterpart in terms of execution time; furthermore, for acceleration, we can exploit Nesterov schemes but we settle with \eqref{eq: projected gradient} for clarity.

\begin{figure}[h]
\centering
\includegraphics[width=.7\linewidth]{sparseHyper2}
\caption{Relative error $\vectornorm{\widehat{\signal} - \bestsignal}_2 / \vectornorm{\bestsignal}_2$ comparison of (\ref{eq:data_fidelity_sparse_simplex}) (Approach 1), (\ref{eq:reg_data_fidelity_sparse_simplex}) (Approach 2) and (\ref{eq:BP}) (Approach 3) as a function of $\numsam$. Each point corresponds to the median value of 30 Monte-Carlo realizations.}
    \label{fig:SparseHyper}
\end{figure}

==> measurelearn.tex <==
\vspace{-2mm}
\subsection{Learning sparse distributions}
\paragraph{Parametric estimation:} As an interesting example, we consider the kernel setting: Let ${\bf x}^{(1)}, {\bf x}^{(2)},\dots, {\bf x}^{(n)} \in \mathbb{R}^{\dimension}$ be an $n$-size corpus of $\dimension$-dimensional samples, drawn from an unknown probability density function (pdf) $p({\bf x})$. 
% SRB; there were some ^\ast and ^\star here for beta, but I think we want \hat instead
Let us form an estimator 
%$\hat{p}({\bf x}) := \sum_{i=1}^n \entry_i^{\star}  
$\hat{p}({\bf x}) := \sum_{i=1}^n \entry_i % here, neither ast nor star nor hat
\kappa_{\sigma}({\bf x}, {\bf x}^{(i)}) $, 
where $\kappa_{\sigma}({\bf x}, {\bf y}) $ is a Gaussian kernel with parameter $\sigma$. 
Let us choose $\hat{p}({\bf x})$ to minimize the integrated squared error criterion: $\text{ISE} = \mathbb{E}\vectornorm{\hat{p}({\bf x}) - p({\bf x})}_2^2$. Hence, the density learning problem becomes learning a weight vector $\bestsignal \in \Delta_{1}^{+}$. The resulting problem can be written as follows \cite{kim1995least,bunea2010spades}
\begin{align}
\bestsignal \in \argmin_{\signal \in \Delta_1^{+}} \left\{ \signal^T \boldsymbol{\Sigma} \signal - {\bf c}^T \signal\right\}, \label{eq:SDE}
\end{align}
where $\boldsymbol{\Sigma} \in \R^{n \times n}$ with $\Sigma_{ij} = \kappa_{\sqrt{2}\sigma}({\bf x}^{(i)}, {\bf x}^{(j)})$, and \begin{align}
c_i = \frac{1}{n - 1}\sum_{j \neq i}\kappa_{\sigma}({\bf x}^{(i)}, {\bf x}^{(j)}), ~\forall i, j.
\end{align}

%While the term $-{\bf c}^T \signal$ induces sparsity in the solution for $\entry_i \geq 0, \forall i$, $\bestsignal$ may not be sparse enough. 
While the combination of the $-{\bf c}^T \signal$ term and the non-negativity constraint induces some sparsity, it may not be enough. 
To avoid overfitting or obtain interpretable results, one might control the level of solution sparsity \cite{bunea2010spades}. In this context, we extend \eqref{eq:SDE} to include cardinality constraints, i.e.~$\bestsignal \in \Delta_{1}^{+} \cap \constraint$. 
%\tasos{Not sure about the kernel matrix satisfying RIP - have to search about it - i cannot find something for the time being}

\paragraph{Non-parametric estimation:}  %We consider discrete setting without loss of generality. 
%Let us assume a random variable ${\bf x}$ takes on a finite values from a set  
%\srbmargin{How is this wlog? I'm changing it}
Let ${\bf x}$ be a discrete random variable taking values in the set   
$\{\boldsymbol{\alpha}_1,\ldots,\boldsymbol{\alpha}_n\}\subseteq \mathbb{R}^\dimension$. The distribution of ${\bf x}$ is characterized by $\signal$, with Prob$({\bf x} = \boldsymbol{\alpha}_i)=\entry_i$, hence $\signal \in \Delta_1^+$.
%. Here, we obviously have $\signal \in \Delta_1^+$.  

Prior information on $\signal$ can be expressed as linear equality constraints, i.e., $\obs=\linmap(\signal)$ as in \eqref{eq: loss function}. For instance, given a function $f:\mathbb{R}^\dimension\rightarrow \mathbb{R}$, $\mathbb{E}f(\cdot) =\sum_{i=1}^n f(\boldsymbol{\alpha}_i)\entry_i$ is a linear measurement.  Moreover, for $\mathcal{C} \subseteq \mathbb{R}^\dimension$, we have Prob$( {\bf x}\in \mathcal{C}) = {\bf c}^T\signal$, where $c_i = 1$ if $\boldsymbol{\alpha}_i \in \mathcal{C}$ and $c_i = 0$  otherwise. For another set $\mathcal{D} \subseteq \mathbb{R}^\dimension$, we can use conditional probabilities to form linear equalities: $({\bf c}-\text{Prob}({\bf x}\in\mathcal{C}~|~{\bf x}\in\mathcal{D}){\bf d})^T\signal = 0$, where $c_i = 1$ if $\boldsymbol{\alpha}_i \in \mathcal{C}\cup  \mathcal{D}$ and $c_i = 0$  otherwise; and, $d_i = 1$ if $\boldsymbol{\alpha}_i \in \mathcal{D}$ and $d_i = 0$  otherwise. 

Since the prior information can be noisy, it makes sense to use the criteria in \eqref{eq: loss function}. The sparsity constraint then allows us to identify the heavy hitters in the distribution (akin to the heavy hitters in a data stream). Moreover, if the linear map is designed so that it has a sub-Gaussian distribution, then one can show that the RIP assumption is satisfied with high probability if the number of rows grow proportional to $k\log\dimension$. 




==> portfolio.tex <==
\subsection{Portfolio optimization} \label{sec:portfolio}
Given a sample covariance matrix $\boldsymbol{\Sigma}$ and expected mean $\boldsymbol{\mu}$, the return-adjusted Markowitz mean-variance (MV) framework selects a portfolio $\bestsignal $ such  that
$
\bestsignal \in \argmin_{\signal \in \Delta_1^{+}} \left\{ \signal^T \boldsymbol{\Sigma} \signal - \tau\boldsymbol{\mu}^T \signal\right\},
$
where $\Delta_1^{+}$ encodes the normalized capital constraint, and $\tau$ trades off risk and return \cite{demiguel2009generalized,brodie2009sparse}. The solution $\bestsignal \in \Delta_1^{+}$ indicates the fractional investments over the $\dimension$ available assets. 

\newcommand{\bsd}{\boldsymbol{\delta}_{\signal}}
While such solutions construct portfolios from scratch, a more realistic scenario  
is to  
%requires to  % ungrammatical
incrementally adjust an existing portfolio as the market changes. Due to costs per transaction, we naturally introduce cardinality constraints. 
In mathematical terms, let $\bar{\signal} \in \mathbb{R}^{\dimension}$ be the current portfolio selection. Given $\bar{\signal}$, we seek to adjust the current selection  $\signal = \bar{\signal} + \boldsymbol{\delta}_{\signal}$ such that $\vectornorm{\boldsymbol{\delta}_{\signal}}_0 \leq k$.  %As a result, 
This leads to the following problem: %$\boldsymbol{\delta}_{\signal}^\ast \in $
\begin{align}\label{exp2:eq:1}\nonumber 
    \bsd^\ast \in
%\argmin_{\bsd: \bsd\in \Sigma_\sparsity \cap \Delta_\lambda} \left[ (\bar{\signal} + 
\argmin_{\bsd\in \constraint \cap \Delta_\lambda} %\left[ 
(\bar{\signal} + 
\bsd)^T \Sigma (\bar{\signal}+ \bsd )- \tau \mu^T (\bar{\signal}+ \bsd), %\right],
\end{align} where $\lambda$ is the level of update, and $k$ controls the transactions costs. During an update, $\lambda=0$ would keep the portfolio value constant while $\lambda>0$ would  increase it. To control the size of the short positions, one can add Tikhonov regularization $\|\bsd\|_2^2$ to the objective. 


%Numerous approaches have been proposed in the literature to solve this problem; see   \cite{bertsimas2009algorithm, cesarone2011portfolio} and references therein. Most of the investigations on cardinality constrained portfolio optimization focus on finding local solutions using greedy techniques, simulated annealing and evolution methods, genetic algorithms, and branch and bound ideas~\cite{chang2000heuristics, bertsimas2009algorithm, gomez2006hybrid}. % and references therein). % SRB: ungrammatical
%\tasos{To be changed: In Section \ref{sec:experiments}, we demonstrate that our basic algorithm \eqref{eq: projected gradient} is competitive with sophisticated software packages while taking a fraction of their run-time. }
%


==> quantum.tex <==
\subsection{Quantum tomography}
In quantum tomography (QT), we are interested in learning a \emph{density matrix} $\X^{\star} \in \mathbb{C}^{d\times d}$, which is Hermitian (i.e., $(\X^\star)^H = \X^{\star}$), positive semi-definite (i.e., $\X^{\star} \succeq 0$) and, satisfies $\text{rank}(\X^{\star}) = r$ and $\tr(\X^{\star}) = 1$.  The QT measurements $\obs$ satisfy $\obs = \linmap(\X^{\star}) +\boldsymbol{\eta}$, where $(\linmap(\X^{\star}))_i = \tr({\bf E}_i \X^{\star}) + \eta_i$, and $\eta_i$ is  zero-mean Gaussian. The operators ${\bf E}_i$'s are typically the tensor product of the $2\times 2$ Pauli matrices \cite{liu2011universal}. 

%Moreover, 
Recently, \cite{liu2011universal} showed that 
almost all such tensor constructions of $\bigO(rd \log^6 d)$ Pauli measurements satisfy the so-called rank-$r$ restricted isometry property (RIP) for all $\X\in \left\{\X\in\C^{d\times d} :  \X \succeq 0, \text{rank}(\X) \leq r, \|\X\|_*\le \sqrt{r} \|\X\|_F\right\}$: 
\begin{equation}\label{eq: RIP-Pauli}
\left(1-\delta_r\right)\|\X\|_F^2 \leq \|\linmap(\X)\|_F^2 \leq \left(1+\delta_r\right)\|\X\|_F^2,
\end{equation}
where $\|\cdot\|_*$ is the nuclear norm (i.e., the sum of singular values), which reduces to $\tr(\X)$ since $\X \succeq 0$. This key observation enables us to leverage the recent theoretical and algorithmic advances in low-rank matrix recovery from a few affine measurements. 

% Changing, Dec 14 2012
% Stephen's comments: the RIP result from Liu simplifies the proof, but the Quantum Tomo PRL had rigorous results for this (without RIP, so the wording is different: for a fixed low rank state, ... )
%Based on the discussion above, to recover $\X^{\star}$ from $\obs$, the following convex relaxation of the rank regularization has been proposed in~\cite{QuantumTomoPRL}:
The standard matrix-completion based approach to recover $\X^{\star}$ from $\obs$ is the following convex relaxation:
\begin{equation} \label{eq:conventional}
    \minimize_{ \X \succeq 0} \|\linmap(\X) - \obs\|_F^2 + \lambda \|\X\|_*.
\end{equation}
This convex approach is both tractable and amenable to theoretical analysis~\cite{QuantumTomoPRL,liu2011universal}. 
%thanks to the RIP of Pauli measurements. 
As a result, we can provably reduce the number of samples $\numsam$  to $ \tilde{\mathcal O}(rd)$ from $\bigO(d^2)$ \cite{liu2011universal}. 
%\tasos{what is the tilde over the big-oh notation?}

Unfortunately, this convex approach fails to account for the physical constraint $\|\X\|_*=1$. To overcome this difficulty, the relaxation parameter $\lambda$ is tuned to obtain solutions with the desired rank followed by normalization to heuristically meet the trace constraint. 

In Section \ref{sec:experiments}, we demonstrate that one can do significantly better via the non-convex algorithm based on \eqref{eq: projected gradient}. A key ingredient then is the following projection:  
\begin{equation}\nonumber
\widehat{\bf B} \in \argmin_{{\bf B} \succeq 0} \vectornorm{{\bf B} - {\bf W}}_F^2~\text{s.t.}~\text{rank}({\bf B}) = r,~\text{tr}({\bf B}) = 1, 
\end{equation}
for a given \emph{Hermitian} matrix ${\bf W} \in \mathbb{R}^{n \times n}$. Since the RIP assumption holds here, we can obtain rigorous guarantees based on a similar analysis to \cite{garg2009gradient,foucart2010sparse, SVP}.

% SRB changing this:
To obtain the solution, we compute the eigenvalue decomposition ${\bf W}={\bf U}{\Lambda}_{\bf W}{\bf U}^H$ and then use the unitary invariance of the problem to  solve $ {\bf D}^\star \in \argmin_{\bf D} \|{\bf D}-{\bf \Lambda}_{\bf W}\|_F$  subject to $\|{\bf D}\|_* \le 1$ and $\text{rank}({\bf D}) \le r$, and from ${\bf D}^\star$ form ${\bf U}{\bf D}^\star {\bf U}^H$ to obtain a solution.
In fact, we can constrain ${\bf D}$ to be diagonal, and thus reduce the matrix problem  to the vector version for ${\bf D} = \text{diag}({\bf d})$, where the projector in Problem \ref{problem:positive} applies. This reduction follows from the  well-known result:
%To obtain the solution, we compute ${\bf W}={\bf U}{\Lambda}_{\bf W}{\bf U}^H$ and then solve $ {\bf D}^\star \in \argmin_{\bf D} \|{\bf D}-{\bf \Lambda}_{\bf W}\|_F$  subject to $\|{\bf D}\|_* \le 1$ and $\text{rank}({\bf D}) \le r$ with the additional constraint that ${\bf D}$ is a diagonal matrix. From ${\bf D}^\star$ we form ${\bf U}{\bf D}^\star {\bf U}^H$ to get a solution. The matrix problem can be reduced to the vector version for ${\bf D} = \text{diag}({\bf d})$, where the projector in Problem \ref{problem:positive} applies. This reduction follows from the  well-known result:

\begin{proposition}[\cite{mirsky1960symmetric}] \label{prop:1}
Let ${\bf A},{\bf B} \in \Rmn$ and $q=\min\{m,n\}$. Let $\sigma_i({\bf A})$ be the singular values of ${\bf A}$ in descending order (similarly for ${\bf B}$). Then,
$$ \sum_{i=1}^q \bigl(\sigma_i({\bf A}) - \sigma_i({\bf B})\bigr)^2  \le \|{\bf A}-{\bf B}\|_F^2. $$
\end{proposition}
The nuclear norm ball is compact and the intersection with the rank constraint also forms a compact set. Hence, via Weierstrauss' theorem, the minimum is achieved at some point, so the solution set is non-empty (as long as $r \ge 1$). As the vector reduction achieves the lower bound, we have the optimal projection onto the physical QT constraints. 

%\srb{This allows us to extend our results for vector projections to matrix projections 
%involving unitarily invariant norms, as has been noticed by 
%\url{http://books.nips.cc/papers/files/nips24/NIPS2011_0061.pdf}
%``Penalty Decomposition Methods for Rank Minimization'', Lu and Zhang, NIPS 2011.
%Their proof is here: \url{http://people.math.sfu.ca/~zhaosong/ResearchPapers/pd-rank.pdf}.
%They use exercise 18 on page 215 of Horn and Johnson. 
%This is what I used in my postNIPS/unitaryInvariantMinimization.pdf file. I think my writeup
%is more concise, but theirs is published. }

